K-D Bonsai: ISA-Extensions to Compress K-D Trees for Autonomous Driving Tasks

Autonomous Driving (AD) systems extensively manipulate 3D point clouds for object detection and vehicle localization. Thereby, efficient processing of 3D point clouds is crucial in these systems. In this work we propose K-D Bonsai, a technique to cut down memory usage during radius search, a critical building block of point cloud processing. K-D Bonsai exploits value similarity in the data structure that holds the point cloud (a k-d tree) to compress the data in memory. K-D Bonsai further compresses the data using a reduced floating-point representation, exploiting the physically limited range of point cloud values. For easy integration into nowadays systems, we implement K-D Bonsai through Bonsai-extensions, a small set of new CPU instructions to compress, decompress, and operate on points. To maintain baseline safety levels, we carefully craft the Bonsai-extensions to detect precision loss due to compression, allowing re-computation in full precision to take place if necessary. Therefore, K-D Bonsai reduces data movement, improving performance and energy efficiency, while guaranteeing baseline accuracy and programmability. We evaluate K-D Bonsai over the euclidean cluster task of Autoware.ai, a state-of-the-art software stack for AD. We achieve an average of 9.26% improvement in end-to-end latency, 12.19% in tail latency, and a reduction of 10.84% in energy consumption. Differently from expensive accelerators proposed in related work, K-D Bonsai improves radius search with minimal area increase (0.36%).

==> figures/__pointcloud_example.tex <==
\begin{figure}[ht]%
\centering
\subfloat[\centering Superior view.]{\label{fig:pointcloudExampleSuperior}\includegraphics[width=0.20\textwidth]{figures/pc_example_superior_white.png}}%
\subfloat[\centering Isometric view.]{\label{fig:pointcloudExampleIso}\includegraphics[width=0.20\textwidth]{figures/pc_example_iso_white.png}}%
\caption{An example of a point-cloud obtained with \gls{LiDAR}. Data from \cite{tierIV2020autowareData}.}%
\label{fig:pointCloudExample}%
\end{figure}

==> figures/__radius_search_share.tex <==
\begin{wrapfigure}{R}{0.21\textwidth}
\includegraphics[width=1.0\linewidth]{figures/radius_search_share.pdf}
\caption{\rebuttal{\textit{Radius search} execution share in two important Autoware.ai tasks.}}
\label{fig:radius_search_share}
\end{wrapfigure}

==> tables/fp_format_impact_on_error.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[htb]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}lrrr@{}}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{ieee\_float\_16}} & \multicolumn{1}{c}{\textbf{b\_float\_16}} & \multicolumn{1}{c}{\textbf{custom\_float\_24}} \\ \midrule
Observed Mistakes             & 28821                                        & 229803                                    & 110                                            \\
Possible Mistakes             & 140440                                       & 1155917                                   & 586                                            \\
Misclassified Points {[}\%{]} & 0.076\%                                      & 0.61\%                                    & 0.0003\%                                       \\
Re-issued in 32-bits {[}\%{]} & 0.37\%                                       & 3.05 \%                                   & 0.0015\%                                       \\
Total Queries Evaluated       & \multicolumn{3}{r}{37,862,020}                                                                                                            \\ \bottomrule
\end{tabular}%
}
\caption{Impact of accuracy in radius search using different floating-point representations for points inside leaves.}
\label{tab:fp_format_impact_on_error}
\end{table}
